ReelCache: An Efficient KV Cache Compression and Management System for Multi-Round Video Generation

Autoregressive video diffusion models produce large KV caches during multi-round video generation. Keeping all these KV chunks would consume substantial memory, while rebuilding discarded caches would significantly delay video chunk generation. This paper presents ReelCache, a KV cache compression system for efficient multi-round, long video generation. ReelCache combines an intra-chunk compressor with an inter-chunk cache manager. The compressor applies low-rank decomposition across channels and video coding to the resulting coefficients, predicting the decomposition rank per transformer layer online to meet retained-energy targets. The cache manager shares basis directions across consecutive chunks and organizes chunk states in a tree, allowing generation branches to share historical state while supporting restoration for resume, rewind, and fork. Experiments across five video generation models show that ReelCache reduces KV storage by 14.46-21.13x relative to baselines and accelerates next-chunk generation by 1.25-3.36x, with less than 1% drop in six representative VBench metrics. GitHub: https://github.com/Tianyu9748/ReelCache

==> tmp/design.tex <==
\section{System Design}
\label{s:design}

\lnote{In this paper, we propose XXX, a KV cache management framework that allow video generation systems to efficiently reuse KV cache to expedite their video generation efficiency. Describe the system workflow, including a inner-chunk KV cache algo, a inter-chink KV cache management, and cross-node KV cache xxx.}

We present \systemname, a KV cache management framework that lets an autoregressive video diffusion system keep the clean KV cache of every generated chunk and reuse it later.
When a user resumes a paused rollout, rewinds to an earlier moment, or forks an
alternative continuation, \systemname restores the historical cache instead of
recomputing it from the clean latents (\S\ref{s:motivation}).
The retained state must be small enough to keep many snapshots per session,
and restoring it must be cheaper than recomputing it.
\systemname has two components.
An \emph{intra-chunk} compressor removes inter-channel redundancy with an SVD
and intra-channel redundancy with a video codec, and it adaptively sets ranks for KVs to meet a per-model energy target(\S\ref{ss:design_intra}).
An \emph{inter-chunk} manager organizes chunk states as a tree in which chunks might inherit the parent's basis if that basis already fits (\S\ref{sec:method-reuse}).
Both components use the same quality criterion, the fraction of a matrix's energy that its stored representation retains.

\subsection{Overview and Workflow}
\label{ss:design_overview}

\phfig{System overview. Commit path (top): clean pass $\rightarrow$ capture pre-RoPE K and V $\rightarrow$
project onto the inherited basis and certify the retained energy $\rightarrow$ share, augment with new directions, or refit $\rightarrow$
encode coefficients on the CPU $\rightarrow$ publish the node into the state tree.
Restore path (bottom): resume / rewind / fork selects a node $\rightarrow$ hot history reused,
other chunks decoded by NVDEC $\rightarrow$ $PQ$ reconstruction and re-RoPE $\rightarrow$ native KV cache, one layer ahead of compute.}

\noindent\textbf{Where \systemname attaches.}
After an AR-DiT denoises chunk $c$, \systemname writes the chunk's keys and values into the cache read by later chunks.
For every layer, it captures the Key after the key normalization and
\emph{before} the rotary position embedding (pre-RoPE K,
\S\ref{ss:motivation_svdcodec}), together with the Value.
Each captured tensor is a matrix $A\in\mathbf{R}^{N\times C}$, where
$N=F\,h\,w$ counts the tokens of the chunk's $F$ latent frames with height $h$ and width $w$, and
$C=H\,D$ counts the channels of $H$ heads of dimension $D$.
The denoising loop is unchanged, and the next chunk still reads the engine's
native in-window cache, so compression stays off its critical path.

\noindent\textbf{Commit path.}
For each matrix, \systemname first projects the new chunk onto the basis
inherited from its parent node and measures how much of its energy that basis
retains (\S\ref{sec:method-reuse}).
If the inherited basis suffices, the chunk shares it and stores only
coefficients.
If it falls short, \systemname adds the few directions the chunk is missing,
or fits a fresh basis when that would be cheaper (\S\ref{ss:design_intra}).
The coefficients are then encoded by a video codec on the CPU.
Once every packet of the chunk is encoded, \systemname atomically publishes
the chunk as an immutable node of the session's state tree.
Only complete clean chunks are published, never a mid-denoising state.

\noindent\textbf{Restore path.}
A resume, rewind, or fork names a node of the tree.
\systemname then materializes the history that the model attends to from that
node.
Chunks still resident on the GPU are reused directly.
The others are decoded by the GPU's hardware video decoder (NVDEC),
multiplied by their basis, re-rotated with RoPE at their original positions,
and written into the engine's native cache layout.
Restoration proceeds layer by layer, one layer ahead of the forward pass.

%------------------------------------------------------------------------------
\subsection{Intra-Chunk KV Compression Pipeline}
\label{ss:design_intra}

\noindent\textbf{Factorization.}
For each layer and target $t\in\{\mathrm{K},\mathrm{V}\}$, \systemname factors
$A\approx PQ$, with a basis $Q\in\mathbf{R}^{r\times C}$ of orthonormal rows and
coefficients $P=AQ^{\top}\in\mathbf{R}^{N\times r}$.
The basis spans the leading right singular vectors of $A$, and the coefficients are projected with that stored basis.

\noindent\textbf{Why SVD before the video codec.}
The two stages remove different redundancies (i.e., inter-channel and intra-channel), and only this order lets both work (\S\ref{ss:motivation_svdcodec}).
The SVD removes the correlation across channels, which a codec cannot see
because it compresses each channel separately.
What remains is a small number of coefficient columns, and each column is still
a smooth field over the chunk's $F\times h\times w$ latent positions, which is
the signal a video codec is built for.
The reverse order applies the SVD to a structured bitstream produced by the video codec, whose syntax must be preserved for decoding.
For example, an HEVC Annex-B bitstream contains start-code prefixes such as \texttt{00 00 01}.
Applying truncated SVD directly to these encoded bytes would approximate their values without preserving their syntactic meaning, causing decoding failures.
In our tests, none of the bitstreams reconstructed from SVD can be decoded successfully.
Therefore, we first factor the KV matrix using SVD and then encode its coefficients, ensuring that the stored coefficient bitstream remains codec-compliant.


\noindent\textbf{Workload placement.}
The projection, the sketches, and the fits run on the GPU over tensors the clean pass has just produced.
Encoding runs on NVENC if available. Otherwise, itw runs on a CPU worker pool.
Either encoding method won't compete with ongoing video denoising for the GPU.
At restore time, NVDEC decodes the coefficients on hardware separate from the GPU's compute units.
For each layer, \systemname dequantizes the decoded coefficients, computes $PQ$, applies RoPE to the Key, and writes the result into the KV cache pool.
Two decoder sessions restore a layer's K and V concurrently, and the next layer is decoded while the current layer computes.


\subsection{Energy-Targeted Online Rank Selection}
\noindent\textbf{Energy-targeted rank.}
The rank a matrix needs varies widely across layers, prompts, and models (\S\ref{ss:motivation_rank}), so one rank for all KV either wastes storage on easy matrices or damages hard ones.
\systemname instead takes a per-target energy target $E_t$ as its quality knob
and tries to store KV with the minimum rank that retains the targeted energy,
\begin{equation}
  r^{\star} = \min\Big\{ r : \textstyle\sum_{i\le r}\sigma_i^{2} \ge E_t\,\|A\|_F^{2} \Big\},
  \label{eq:rank}
\end{equation}
where $\sigma_1\ge\sigma_2\ge\dots$ are the singular values of $A$.
The targets are chosen once per model from an energy-quality profile
(\S\ref{ss:motivation_rank}). 
\tianyu{Figures to show the quality-energy tradeoff for all models in Appendix.}
In \systemname, we use $E_{\mathrm{K}}{=}0.98$ and $E_{\mathrm{V}}{=}0.95$.
% Stored ranks are rounded up to multiples of 32, which reduces the number of distinct tensor shapes seen by the batched kernels and the codec.
% Also, it reduces the prediction difficulty that \systemname only needs to estimate the bucket, instead of exact rank values. 
To simplify online rank estimation, \systemname rounds ranks up to multiples of 32 and predicts the corresponding rank bucket rather than an exact rank.
This coarser prediction space reduces the precision required of the estimator, at the cost of storing up to 31 additional directions relative to the unrounded rank.
% As a secondary benefit, bucketing limits tensor-shape diversity, which can make the inputs to batched kernels and the codec more consistent.

\noindent\textbf {Select the rank without the full spectrum.}
Evaluating Eq.~(\ref{eq:rank}) exactly through a dense Gram decomposition requires an $O(NC^2)$ matrix product followed by an $O(C^3)$ eigen decomposition, where $N$ and $C$ are the token count and channel width.
\systemname~avoids this full-spectrum computation by exploiting the similar relative shapes of rank--energy curves within a layer.

Figure~\ref{fig:rank-energy-pattern} shows the cumulative energy across prompts over ranks for CausVid layers 15 and 25.
Within each layer, prompts differ substantially in the energy captured by the first few singular directions, as highlighted by the red box.
At larger ranks, the absolute gaps in captured energy narrow, and the spectral tails exhibit approximately similar relative decay patterns.
\tianyu{Report the across-prompt captured-energy spread at ranks 1 and 128 for each layer and matrix type, in percentage points.}
This observation suggests that an estimator can learn the typical rank--energy relationship of a layer and reuse it across prompts.
We choose a power-law approximation because it describes progressively diminishing energy gains with few parameters and turns rank prediction into an inexpensive linear regression in logarithmic coordinates.
Unlike learning an entire curve, this formulation requires only a scale and an exponent, which can be updated online from verified fits.
The remaining question is how to determine where an incoming K$|$V lies on that relationship without computing its full spectrum.

\noindent\textbf{Obtain the anchor from a small-rank basis.} 
Within each layer, the contributions of successive singular directions diminish in a similar pattern after the leading directions.
However, the energy captured by those leading directions varies across prompts.
A small-rank measurement provides a solid anchor: it tells the estimator how much energy has already been captured, so the learned decay pattern can guide prediction of the rank needed to reach the target.
Hence, \systemname constructs a column-orthonormal, $m$-direction sketch $S_m$ of $X$ (e.g., $m$=32), and measures its captured-energy fraction:
 \begin{equation}
   \hat E_m
   =\frac{\|XS_m\|_F^2}{\|X\|_F^2}
   =\frac{\operatorname{tr}\big((XS_m)^\top(XS_m)\big)}
          {\|X\|_F^2}.
   \label{eq:rank-anchor-energy}
 \end{equation}
If $\hat E_m\ge E_t$, the sketch already meets the fitting target and supplies the first rank bucket.
Otherwise, \systemname extrapolates from this anchor.

\noindent\textbf{Predict the rank from the anchor.}
We approximate the energy-captured trajectory as:
\begin{equation}
  E_X(r)
  \approx 1-\big(1-E_X(m)\big)
                 (r/m)^{-\gamma_{\ell t}},
  \qquad r\ge m
  \label{eq:rank-energy-model}
\end{equation}
where $E_X(r)$ denotes the energy fraction captured by the optimal rank-$r$ approximation, $\gamma_{\ell t}>0$ describes the decay pattern for layer $\ell$ and target $t$.
Substituting the sketch measurement for $E_X(m)$ and solving for
the rank at which the captured energy reaches $E_t$ gives
\begin{equation}
  \hat r
  \approx m\left(
    \frac{1-\hat E_m}{1-E_t}
  \right)^{1/\gamma_{\ell t}}
  \label{eq:rank-anchor-prediction}
\end{equation}
Taking logarithms motivates a learned log-linear estimator:
\begin{equation}
  \ln\hat r
  \approx \ln m
  \!+\!\frac{1}{\gamma_{\ell t}}
  \ln\!\frac{1-\hat E_m}{1-E_t}
  =a_{\ell t}
  \!+\!b_{\ell t}\ln\!\frac{1-\hat E_m}{1-E_t}
  \label{eq:rank-online-line}
\end{equation}
In the online estimation, both coefficients $a_{\ell t}$ and $b_{\ell t}$ are learned from verified fits to accommodate layer-specific behavior and sketch approximation error.
 
\noindent\textbf{Verify the prediction and update the predictor.}
\systemname fits a subspace at the predicted rank bucket and checks its captured energy.
If the target is not met, it adds an extra bucket of directions (i.e., 32 in \systemname) and repeats the check until meeting the target.
It also checks if it can trim buckets of directions by ordering the fitted subspace based on captured energy.
The verification stage supplies training data for the predictor without a full-spectrum computation.
We then update the predictor with these training data during online estimation. 
We use the unrounded exact rank value, $r_{\mathrm{exact}}$, as the label, so bucket rounding doesn't inflate the learned rank.
For fits requiring more than the anchor rank $m$, let
$x=\ln\big((1-\hat E_m)/(1-E_t)\big)$ and
$\mathbf z=(1,x)^\top$.
Each layer maintains its online regression state,
initialized with $\mathbf M=2I_2$ and
$\mathbf v=\mathbf M(\ln m,1)^\top$.
After verification, we update coefficients $(a_{\ell t},b_{\ell t})$ as:
\begin{equation}
  \begin{aligned}
    & \mathbf M=\mathbf M+\mathbf z\mathbf z^\top, \quad
    \mathbf v=\mathbf v
      +\mathbf z\ln r_{\mathrm{exact}}, \\
    &(a_{\ell t},b_{\ell t})^\top
      =\mathbf M^{-1}\mathbf v
  \end{aligned}
  \label{eq:rank-online-update}
\end{equation}
This update incorporates the verified fit into subsequent predictions, with state retained across prompts.



%------------------------------------------------------------------------------
\subsection{Inter-Chunk KV Cache Management}
\label{sec:method-reuse}

\noindent\textbf{State tree.}
\systemname records a session as a tree of chunk states.
Each node holds, for every layer and target, a block of basis, coefficients, and the metadata needed to restoration: token positions, geometry, codec parameters, energy target, and rank.
An edge connects a chunk to the chunk it was generated after, and the session keeps a pointer to its current node.
Interactive operations become tree operations.
\textbf{Resume} continues from the node.
\textbf{Rewind} moves the head to an ancestor and restores that ancestor's history.
\textbf{Fork} starts a new branch whose first chunk is a child of any existing node and leaves the parent's branch untouched.
Nodes and blocks are immutable, and branches share their common prefix without copying it (i.e., stored once).
Restoring a node reads the nodes on its path to the root that fall inside the model's attention window.

\noindent\textbf{Inherit, certify, augment.}
Consecutive chunks span nearly the same KV subspace, but a similarity score between bases needs the new chunk's own basis and does not tell whether the old basis still fits enough to obtain the target energy (\S\ref{ss:motivation_sharingbasis}).
\systemname therefore never compares bases.
Each branch carries an \emph{active basis} per layer and target, and a new
chunk tests that basis directly on its own data (Algorithm~\ref{alg:commit}).
It projects the chunk onto the stored basis $\tilde Q$ and computes the energy $e$ the reconstruction retains,
\begin{equation}
  P = A\tilde Q^{\top},\qquad R = A - P\tilde Q,\qquad
  e = 1 - \frac{\|R\|_F^{2}}{\|A\|_F^{2}} .
  \label{eq:certify}
\end{equation}
% The test costs two thin products, $O(NCr)$.
% Its projection $P$ is the coefficient that the chunk stores if the basis is kept. 
% On an RTX PRO 6000, the projection-energy test takes 0.115~ms per CausVid's K$|$V, against 14.6~ms for a fresh FP32 fit.
If $e\ge E_t$, the chunk shares the basis and keeps only the shortest prefix of it that reaches the target.
Otherwise the residual $R$ holds exactly what the basis misses, and
\systemname runs \textsc{Fit} on it for the remaining fraction:
\begin{equation}
  U = \textsc{Fit}\Big(R,\ \frac{E_t - e}{1 - e}\Big)
  \label{eq:augment}
\end{equation}
\systemname re-orthogonalizes the new directions against $\tilde Q$, and appends them to
the active basis.
The chunk stores its coefficients on the extended basis and only the new basis
rows.
A shared chunk and an augmented chunk therefore meet the same energy target as
a freshly fitted one, and a fresh fit is the special case of an empty active
basis.

\begin{algorithm}[t]
\caption{Commit matrix $A$ of a new chunk, given the branch's active basis $Q$.}
\label{alg:commit}
\begin{algorithmic}[1]
\small
\STATE $P \leftarrow A\tilde Q^{\top}$,\quad $R \leftarrow A - P\tilde Q$ \hfill // project
\STATE $e \leftarrow 1-\|R\|_F^{2}/\|A\|_F^{2}$ \hfill // certify
\IF{$e \ge E_t$}
  \STATE keep the shortest prefix of $Q$ reaching $E_t$ \hfill // share
\ELSE
  \STATE $U \leftarrow \textsc{Fit}\big(R,\ (E_t-e)/(1-e)\big)$ \hfill // new directions
  \IF{storing $[\,Q,U^{\top}]$ costs more than a fresh fit}
    \STATE $Q \leftarrow \emptyset$,\quad $U \leftarrow \textsc{Fit}(A, E_t)$ \hfill // refit
  \ENDIF
  \STATE $Q \leftarrow [\,Q, \ U^{\top}]$ \hfill // augment
\ENDIF
\STATE $P \leftarrow A\tilde Q^{\top}$ // encode $P$ with HEVC and store the new basis
\end{algorithmic}
\end{algorithm}

\noindent\textbf{When to refit.}
Each augmentation adds coefficient columns to every later chunk that inherits the extended basis, so the active basis cannot grow forever.
\systemname refits a fresh basis when the augmented representation would store more bytes than a fresh fit.
It estimates the fresh rank from the layer's most recent fit, because a layer's rank changes little between consecutive chunks.
Refits thus split a rollout into groups of chunks that grow one basis, much as intra frames split a video into groups of pictures.
A scene cut or a large motion needs many new directions and triggers a refit through the same rule, with no separate detector.
A fork inherits the active basis of the node it branches from, so sibling branches extend a common basis independently, and their shared rows are stored once.

% \noindent\textbf{Why augmentation.}
% Augmentation spends its bytes exactly on the child's new content.
% In a CausVid study with 32 chunk transitions, augmentation added fewer than 20 directions per matrix on average.
% Compared with a fresh basis per chunk at the same energy target, it changed next-chunk SSIM by $-0.005$ on average and, under our codec byte model, stored about half the bytes (\S\ref{sec:eval}).
% Sharing every basis without a check lost 0.033 SSIM on average and up to 0.213 across a scene cut.


\noindent\textbf{Random access per node.}
Each node's coefficients form an independent codec stream, so any node can be decoded without its neighbors, as rewind and fork require.
Only the basis rows are shared.
Group several nodes' coefficients and codec encode this group as one stream would be only slightly smaller.
For example, with one Key basis shared by six consecutive CausVid chunks, joint codec encoding these six coefficients reaches $35.4\times$ against $33.2\times$ for per-coefficient codec encoding.
But decoding one node's codec stream (i.e., encoded coefficient) would then require decoding its predecessors in the same group, so \systemname gives up this small gain for random access.

% \noindent\textbf{Residency.}
% The compressed nodes in host memory, backed by a persistent store, are the
% source of truth.
% On top of them, each GPU keeps a budgeted hot tier of decoded, attention-ready
% history for its active sessions and evicts the oldest chunks first.
% A restore uses hot copies where they exist and decodes only the rest.


==> tmp/motivation.tex <==
% Draft of Background & Motivation and Challenges & Observations (2026-09-29).
% Drop-in replacement for tex/motivation.tex: use \input{tmp/motivation} instead of \input{tex/motivation}.
% MAGI-1 removed. Recomputation and storage use LongLive 2.0, RAVEN, SkyReels-V2-DF, and CausVid.
% LongLive 2.0 is used instead of LongLive 1.0 because its rebuild takes longer (17.6 s vs 6.1 s at 32 history chunks).
% Figures and their data/scripts: tmp/figs/ (make_motivation_figs.py regenerates the three new plots).
% Labels kept from tex/motivation.tex: s:motivation, s:challenge, ss:motivation_svdcodec, fig:lowrank,
% tab:svdcodec-pipeline, ss:motivation_sharingbasis, fig:basisoverlap. The SP subsection is removed.

\section{Background and Motivation}
\label{s:motivation}

\noindent\textbf{Autoregressive video generation.}
Modern video diffusion systems synthesize videos by iteratively denoising latent
representations conditioned on text prompts and, optionally, reference images or videos.
We focus on autoregressive video diffusion models, such as
CausVid~\cite{causvid}, LongLive~\cite{longlive,longlive2.0}, RAVEN~\cite{raven}, and
SkyReels-V2~\cite{skyreels-v2}, which generate a video chunk by chunk.
For each chunk, a diffusion transformer refines noisy latent tokens while attending to
the keys and values (KV) of previously generated chunks, which keeps the video
temporally consistent.
After a chunk is denoised, the model runs one more forward pass on the clean latents
(timestep zero) and writes the chunk's keys and values into the KV cache that later
chunks read.
A variational autoencoder decodes the latents into RGB frames.
Generation need not proceed as a single uninterrupted request: interactive workflows
update prompts, revisit earlier content, or explore alternative continuations from a
shared prefix~\cite{longlive,longlive2.0,worldmodel}.
Resuming, rewinding, and forking all need the historical KV cache of the point they
continue from.

\noindent\textbf{Recomputing historical KV wastes computation and increases latency.}
When the historical KV cache is not available, the server must rebuild it before it can
denoise the next chunk.
An exact rebuild replays the clean forward pass of every committed chunk in order,
because each chunk's keys and values depend on the cache it attended to when it was
committed.
This holds even for models that attend to a bounded window, so the rebuild grows with
the length of the history rather than with the size of the window.
Figure~\ref{fig:recompute} measures the latency of generating the next chunk on an
RTX PRO 6000 GPU, with the history cache resident and with it rebuilt from the stored
clean latents.
The rebuilt caches are bit-identical to the resident ones, so the extra time is pure
recomputation.
For LongLive 2.0 at $1280{\times}704$, the next chunk takes 2.4~s with the cache
regardless of how long the history is, but 3.9~s after rebuilding 5~s of history and
17.6~s after rebuilding 43~s ($7.4\times$), of which the rebuild is 87\%.
RAVEN attends to its full history, so even its cached latency grows, from 0.57~s to
3.6~s at 16~s of history, and rebuilding raises it to 18.1~s ($5.0\times$).
CausVid behaves the same way: at 16~s of history, the next chunk takes 2.1~s with the
cache and 11.5~s after rebuilding ($5.5\times$).
% CausVid: latency_prefix_cache_20260927/causvid/rtx6000_blackwell-job-interactive-gpu-n79/latency.csv
% (same RTX PRO 6000 model; 3 reps; rebuild bit-exact). Beyond 6 history chunks CausVid attends over more
% than its trained 21-latent-frame context; this changes quality, not the timing.
SkyReels-V2-DF (14B, $1280{\times}720$, classifier-free guidance with two cached
branches) is so large that a single 96~GB GPU cannot hold more than one block (0.8~s)
of its history (Figure~\ref{fig:kvstorage}).
On four A100 GPUs with sequence parallelism~\cite{ulysses}, rebuilding 5~s of its
history takes 27.2~s on top of 69.5~s of denoising, a 39\% increase.
% SkyReels: paper/native_sp_inference_20260912/report.md (4x A100-80GB, 30 one-latent-frame blocks = 121 frames,
% 50 UniPC steps, CFG 6); single RTX PRO 6000: one 5-frame block rebuilt in 6.7 s, OOM with two blocks.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{tmp/figs/fig_recompute_latency.pdf}
\vspace{-6mm}
\caption{Next-chunk latency with the history KV cache resident (solid) and rebuilt from
the stored clean latents (dashed), on an RTX PRO 6000. History length is in seconds of
video at 24~FPS. Text encoding and VAE decoding are excluded.}
\label{fig:recompute}
\end{figure}

Existing frameworks provide model-specific KV caching for ongoing
generation~\cite{vllm-omni,sglang,diffusers,xdit}, but maintaining the active context is
distinct from preserving historical checkpoints for later reuse.
In window-bounded configurations, KV entries outside the retained context are evicted.
If a later rollback or alternative continuation requires an evicted state and no saved
copy exists, the server must rebuild the required history.
Caching the active window alone therefore does not eliminate recomputation across
interactive requests.

\noindent\textbf{Historical KV quickly exhausts memory.}
A straightforward solution is to retain the KV cache beyond the active attention window,
in GPU memory and with CPU offloading as in LLM serving
systems~\cite{lee2024infinigen,liu2025lmcache}.
Video KV, however, is large and grows quickly.
Table~\ref{tab:kvsize} and Figure~\ref{fig:kvstorage} estimate the size of the history
cache in half precision, assuming 24~FPS video.
One second of LongLive 2.0 video produces 1.95~GB of keys and values, and one second of
CausVid or RAVEN video produces 1.73~GB.
SkyReels-V2 produces 35.4~GB per second, because it caches both guidance branches of a
14B model.
Even if an entire 96~GB RTX PRO 6000 held nothing but history, it would fit less than a
minute of LongLive 2.0, CausVid, or RAVEN video and less than 3~s of SkyReels-V2 video.
In practice SkyReels-V2 runs out of memory on this GPU with only two blocks (1.7~s) of
history.
Dedicating 1~TB of host memory raises the limit to about 9~minutes for the smaller models
and 28~s for SkyReels-V2.
These are optimistic upper bounds: they ignore model weights, activations, other tenants,
and the fact that concurrent sessions and alternative branches each need their own history.
Retaining uncompressed historical KV therefore scales poorly beyond a few short videos,
which calls for a more compact representation of reusable video state.


\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{1.3mm}
\caption{Estimated size of the history KV cache (FP16, 24~FPS) and the longest history
that fits in one RTX PRO 6000 (96~GB) or in 1~TB of host memory, ignoring everything else.}
\label{tab:kvsize}
\begin{tabular}{lrrrrr}
\toprule
& \multicolumn{3}{c}{KV size (GB)} & \multicolumn{2}{c}{Longest history} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-6}
Model & 1~s & 1~min & 5~min & 96~GB & 1~TB \\
\midrule
LongLive 2.0 & 1.95 & 117 & 584 & 49~s & 8.6~min \\
RAVEN & 1.73 & 104 & 518 & 56~s & 9.7~min \\
SkyReels-V2-DF & 35.4 & 2{,}123 & 10{,}617 & 2.7~s & 28~s \\
CausVid & 1.73 & 104 & 518 & 56~s & 9.7~min \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{tmp/figs/fig_kv_storage.pdf}
\vspace{-6mm}
\caption{Estimated size of the history KV cache (FP16) as the video grows, at 24~FPS.
CausVid and RAVEN share the same backbone and resolution.}
\label{fig:kvstorage}
\end{figure}

\noindent\textbf{Compressing the KV cache is promising.}
Our basic idea is to compress the historical KV cache.
Both low-rank decomposition and video coding have been shown to compress KV caches
effectively in LLM serving.
ShadowKV~\cite{shadowkv} and Palu~\cite{palu} store keys in a low-rank form, and
LLM.265~\cite{llm265} and KVCodec~\cite{kvcodec} compress KV tensors with standard video
codecs.
The system cost is also favorable for video generation.
GPUs have dedicated hardware video decoders (NVDEC) that restore a codec stream without
using the compute units that generate video, and encoding can run on the CPU without
interfering with generation on the GPU.
However, applying these techniques to the KV cache of video generation raises three
challenges (\S\ref{s:challenge}).

%==============================================================================
% \section{Challenges and Observations}
% \label{s:challenge}

% We characterize historical KV caches to identify how to compress them.
% Because each generated chunk conditions the chunks after it, an error in the restored
% cache can change later outputs, so we evaluate compression by the quality of the decoded
% video (SSIM against uncompressed generation).
% Unless otherwise noted, measurements use CausVid~\cite{causvid} at $832{\times}480$.

% %------------------------------------------------------------------------------
% \subsection{Either Technique Alone Leaves Redundancy}
% \label{ss:motivation_svdcodec}

% Video KV tensors carry two kinds of redundancy.
% Across channels, the keys and values of a chunk lie close to a low-dimensional subspace.
% Figure~\ref{fig:lowrank} shows that 96 singular directions, 6.25\% of the 1536 channels,
% capture 98\% of the energy of the pre-RoPE Key.
% Within each channel, the values form a smooth field over the chunk's frames and spatial
% positions, which is the redundancy a video codec is built to remove.
% A codec compresses each channel separately and cannot see the correlation across
% channels, while an SVD removes that correlation but leaves each coefficient channel
% uncompressed.
% Table~\ref{tab:svdcodec-pipeline} confirms that neither tool alone suffices:
% HEVC alone compresses the pre-RoPE Key by $7.82\times$ and SVD alone by $4.52\times$,
% whereas SVD followed by HEVC on the coefficients reaches $14.12\times$.
% % TODO: the three rows are at different SSIM (0.986 / 0.991 / 0.980); an equal-quality comparison
% % (or a ratio-vs-SSIM curve) would make this claim harder to dispute.

% \begin{figure}[t]
% \includegraphics[width=1\columnwidth]{imgs/motivation/cumulative_energy.pdf}
% \vspace{-8mm}
% \caption{Video KV is low-rank across the channel dimension ($C{=}1536$): a small basis
% captures almost all of the energy.}
% \label{fig:lowrank}
% \end{figure}

% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{3.2mm}
% \caption{Compression ratio and SSIM of pre-RoPE Key compression pipelines (CausVid, one chunk, SVD rank 256).}
% \label{tab:svdcodec-pipeline}
% \begin{tabular}{lcc}
% \toprule
% Method & Ratio & SSIM~$\uparrow$ \\
% \midrule
% HEVC only                              & 7.82$\times$  & 0.986 \\
% SVD only                               & 4.52$\times$  & 0.991 \\
% SVD $\rightarrow$ HEVC (coefficients)  & 14.12$\times$ & 0.980 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \noindent\textbf{Which Key to compress.}
% Models apply the rotary position embedding (RoPE) to keys before caching them, and the
% rotation depends on each token's position.
% Table~\ref{tab:prepost} compares an SVD of the Key taken before RoPE with one taken
% after it, at the same rank and therefore the same compression ratio.
% The pre-RoPE Key gives higher SSIM in 50 of 52 settings across five models, and the gap
% is largest at low rank.
% The two exceptions are SkyReels-V2 at ranks of 1024 and above, where both
% representations are at the model's noise floor.
% We therefore compress the pre-RoPE Key and re-apply RoPE after reconstruction.
% % Source: profiling_summary_20260929 (study A; H = 1 and 2 history chunks; LongLive 1.0 is the fifth model).

% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{1.6mm}
% \caption{SSIM of the next chunk when the history Key is replaced by an SVD at a fixed
% rank, taken before (pre) or after (post) RoPE (one history chunk; Value uncompressed).}
% \label{tab:prepost}
% \begin{tabular}{lcccc}
% \toprule
% & \multicolumn{2}{c}{Rank 64} & \multicolumn{2}{c}{Rank 256} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}
% Model & pre & post & pre & post \\
% \midrule
% LongLive 2.0 & \textbf{0.823} & 0.769 & \textbf{0.924} & 0.885 \\
% RAVEN & \textbf{0.989} & 0.966 & \textbf{0.998} & 0.996 \\
% SkyReels-V2-DF & \textbf{0.815} & 0.745 & \textbf{0.861} & 0.840 \\
% CausVid & \textbf{0.970} & 0.918 & \textbf{0.995} & 0.990 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{observationbox}{Observation One:}
% Video KV has both inter-channel and intra-channel redundancy. Compressing it well needs
% both an SVD across channels and a video codec within channels, applied to the pre-RoPE Key.
% \end{observationbox}

% %------------------------------------------------------------------------------
% \subsection{The Required Rank Varies Widely}
% \label{ss:motivation_rank}

% An SVD keeps the leading $r$ directions of a matrix, and the quality of the video depends
% on how much of the matrix's energy they retain.
% For CausVid over 36 prompts, next-chunk SSIM rises steadily with the retained energy:
% compressing only the Value to 90\%, 95\%, and 98\% of its energy gives SSIM 0.940, 0.976,
% and 0.991, and compressing only the Key to the same levels gives 0.796, 0.895, and 0.955.
% % Source: energy_rank_quality_20260921/analysis/causvid-production-v4-resume-v1/quality_by_energy.csv (svd_only).
% The rank needed to retain a given energy, however, differs widely between matrices
% (Figure~\ref{fig:rankvar}).
% Across the 30 layers of CausVid, retaining 98\% of the Key energy needs a mean rank from
% 1 to 153, and retaining 95\% of the Value energy needs 16 to 269.
% Within a single layer, the rank also changes from prompt to prompt, by a median of 70
% for the Key and 102 for the Value.
% It changes across models as well: 98\% of the Key energy needs a median rank of 111 of
% 1536 channels in LongLive 1.0 but 294 of 3072 in LongLive 2.0.
% % Source: basis_overlap_longlive_20260929/summary/README.md (per-chunk spectra, median over layers, chunks, prompts).
% A single rank for all matrices must cover the hardest one.
% To meet the targets above in every layer and prompt, a uniform rank must be 209 for the
% Key and 333 for the Value, $2.5\times$ and $2.1\times$ the mean rank each matrix actually
% needs.
% % Source: tmp/figs/rank_per_layer_summary.csv (from rank_profiles.csv, 36 prompts).

% \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{tmp/figs/fig_rank_per_layer.pdf}
% \vspace{-6mm}
% \caption{Smallest rank that retains 98\% of the pre-RoPE Key energy and 95\% of the Value
% energy, per layer of CausVid, across 36 prompts. The dashed line is the uniform rank
% that meets the target everywhere.}
% \label{fig:rankvar}
% \end{figure}

% Giving every matrix its own rank requires knowing its spectrum.
% Computing the exact rank means a full eigendecomposition per matrix, whose cost grows
% cubically with the channel count, which reaches 3072 in LongLive 2.0 and 5120 in
% SkyReels-V2, for every layer, for both keys and values, and for every chunk.

% \begin{observationbox}{Observation Two:}
% Video quality follows the retained energy, but the rank needed to retain it varies widely
% across layers, prompts, and models. The rank should be chosen per matrix, without
% computing the full spectrum.
% \end{observationbox}

% %------------------------------------------------------------------------------
% \subsection{Consecutive Chunks Share Subspaces}
% \label{ss:motivation_sharingbasis}

% Consecutive chunks of a video show nearly the same scene, so their KV caches may span
% nearly the same channel subspace.
% We quantify this with the normalized subspace overlap
% \[
%     s(i,j) = \frac{\|Q_i Q_j^{\top}\|_F^2}{r},
% \]
% where $Q_i$ and $Q_j$ are the row-orthonormal rank-$r$ channel bases of chunks $i$ and $j$.
% The score is the mean squared cosine of the principal angles between the two subspaces,
% and it does not depend on the order or sign of the basis vectors.
% Figure~\ref{fig:basisoverlap} shows its distribution for adjacent chunks generated under
% the same prompt, with $r=256$.
% The mean overlap is 0.86--0.89 for both Key and Value in CausVid, LongLive 1.0, and
% LongLive 2.0, compared with 0.71--0.74 for chunks generated from different prompts.
% The raw tensors are less alike: aligned token by token, adjacent LongLive 2.0 chunks have
% a cosine similarity of only 0.76 for the Key and 0.41 for the Value.
% Content moves between chunks, but the channel subspace it lives in stays nearly the same.
% % Sources: basis_overlap_longlive_20260929/summary (6,720 adjacent pairs per target per LongLive model;
% % 32 prompts x 8 chunks); CausVid 600 pairs per target (4 prompts x 6 chunks).

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.85\textwidth]{tmp/figs/fig_overlap_cdf_models.pdf}
% \vspace{-3mm}
% \caption{Subspace overlap of adjacent chunks under the same prompt (solid) and of chunks
% from different prompts (dashed), for the pre-RoPE Key (left) and Value (right), $r=256$.}
% \label{fig:basisoverlap}
% \end{figure*}
% % Optional companion figure (LongLive only): raw token-aligned cosine vs basis overlap,
% % tmp/figs/fig_raw_cos_vs_overlap_longlive.pdf.

% This similarity is valuable because the basis dominates the compressed size of a single
% chunk.
% For one CausVid chunk, the FP16 basis is about 80\% of the Key's compressed bytes.
% When six consecutive chunks share one Key basis, the Key compression ratio rises from
% $9.9\times$ to $33.2\times$.
% % Source: docs/gather_free_kv_svd.md ("Why one chunk caps at ~13x"), per-chunk coefficient coding.
% Sharing blindly is not safe, however.
% Reusing the previous chunk's basis for every matrix, without any check, lowers the next
% chunk's SSIM by 0.033 on average and by up to 0.213 when the prompt changes.
% % Source: basis_similarity_cosine_20260928/video_arm_summary.csv (32 transitions, 8 rollouts).

% The difficulty is deciding when a basis can be shared.
% Similarity scores such as the overlap compare two bases, so they need the new chunk's own
% basis, which is exactly the computation that sharing is meant to avoid.
% They also do not decide the question.
% Two adjacent Key matrices in the same CausVid rollout have the same mean cosine
% similarity (0.267 and 0.268) and nearly the same overlap (0.951 and 0.930).
% Within the bytes of a fresh fit, the previous chunk's basis retains 98.2\% of the energy
% of the first matrix but only 97.6\% of the second, so it meets a 98\% target for one and
% misses it for the other.
% % Source: basis_similarity_cosine_20260928/examples.csv (p003 L4 c3->c4 vs p003 L6 c1->c2).

% \begin{observationbox}{Observation Three:}
% Consecutive chunks span nearly the same KV subspace, so sharing a basis across them can
% remove most of the basis storage. Whether a basis still fits a new chunk must be decided
% from the new chunk's own data, without fitting its basis.
% \end{observationbox}

